Nonlinear Moment Matching for the Simulation-Free Reduction of Structural Systems

This paper transfers the concept of moment matching to nonlinear structural systems and further provides a simulation-free reduction scheme for such nonlinear second-order models. After first presenting the steady-state interpretation of linear moment matching, we then extend this reduction concept to the nonlinear second-order case based on Astolfi [2010]. Then, similar simplifications as in Cruz Varona et al. [2019] are proposed to achieve a simulation-free nonlinear moment matching algorithm. A discussion on the simplifications and their limitations is presented, as well as a numerical example which illustrates the efficiency of the algorithm.

==> auxfiles/algos.tex <==
\begin{algorithm}
	\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
	\SetKwFor{Foreach}{for each}{do}{endfor}
	\SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{endif}
	\Input{A method \emph{m}}
	\Output{result}
	\Foreach { $x \in M_{x}$}{
		do something
	}
	\caption{Algorithm}\label{Method}
\end{algorithm}



==> auxfiles/formulas.tex <==
\begin{definition}
	The Taylor series expansion of the transfer function $\boldsymbol{G}(s)$ around a complex number $\sigma \in \mathbb{C}$, also called \emph{shift} or \emph{expansion / interpolation point}, is given by
	\begin{equation}
		\boldsymbol{G}(s) = \sum_{i=0}^{\infty} \boldsymbol{m}_{i}(\sigma) (s - \sigma)^i\,,
	\end{equation}
	where $\boldsymbol{m}_i(\sigma)$ is called the $i$-th \emph{moment} of $\boldsymbol{G}(s)$ around $\sigma$. The moments represent the Taylor coefficients and satisfy:
	\begin{equation*}
		\begin{aligned}
			\boldsymbol{m}_i(\sigma) = \frac{1}{i!} \left.\left[\frac{\mathrm{d}^{i}}{\mathrm{d}s^{i}} \, \boldsymbol{C}(s^2 \boldsymbol{M} + s \boldsymbol{D} + \boldsymbol{K})^{-1} \boldsymbol{B}\right]\right|_{s=\sigma}. \\[0.5em]
		\end{aligned}
	\end{equation*}
\end{definition}


\begin{align}
\boldsymbol{M} \ddot{\boldsymbol{q}}(t) + \boldsymbol{f}\big(\boldsymbol{q}(t)\big) &= \boldsymbol{B} \boldsymbol{F}(t), \ \boldsymbol{q}(0) \!=\! \boldsymbol{q}_0, \dot{\boldsymbol{q}}(0) \!=\! \dot{\boldsymbol{q}}_0 \nonumber \\
\boldsymbol{y}(t) &= \boldsymbol{h}\big(\boldsymbol{q}(t)\big),
\end{align}
\begin{align}
\boldsymbol{M} \ddot{\boldsymbol{q}}(t) + \boldsymbol{f}\big(\dot{\boldsymbol{q}}(t), \boldsymbol{q}(t)\big) &= \boldsymbol{B} \boldsymbol{F}(t), \ \boldsymbol{q}(0) \!=\! \boldsymbol{q}_0, \dot{\boldsymbol{q}}(0) \!=\! \dot{\boldsymbol{q}}_0 \nonumber \\
\boldsymbol{y}(t) &= \boldsymbol{h}\big(\boldsymbol{x}(t)\big),
\end{align}
\begin{align} \label{eq:nonlin-FOM}
\boldsymbol{M} \ddot{\boldsymbol{q}}(t) + \boldsymbol{D} \dot{\boldsymbol{q}}(t) + \boldsymbol{f}\big(\boldsymbol{q}(t)\big) &= \boldsymbol{B} \boldsymbol{F}(t), \ \boldsymbol{q}(0) \!=\! \boldsymbol{q}_0, \dot{\boldsymbol{q}}(0) \!=\! \dot{\boldsymbol{q}}_0 \nonumber \\
\boldsymbol{y}(t) &= \boldsymbol{h}\big(\boldsymbol{x}(t)\big),
\end{align}

\begin{equation} \label{eq:nonlin-ROM-nonlin-proj}
\begin{aligned}
\frac{\partial \boldsymbol{\omega}(\boldsymbol{q})}{\partial \boldsymbol{q}} \boldsymbol{M} \frac{\partial \boldsymbol{\nu}(\boldsymbol{q}_{\mathrm{r}})}{\partial \boldsymbol{q}_{\mathrm{r}}} \dot{\boldsymbol{q}}_{\mathrm{r}} + \frac{\partial \boldsymbol{\omega}(\boldsymbol{q})}{\partial \boldsymbol{q}} \boldsymbol{M} \frac{\partial^2 \boldsymbol{\nu}(\boldsymbol{q}_{\mathrm{r}})}{\partial \boldsymbol{q}_{\mathrm{r}}^2} \, \dot{\boldsymbol{q}}_{\mathrm{r}} \otimes \dot{\boldsymbol{q}}_{\mathrm{r}} \\ + \frac{\partial \boldsymbol{\omega}(\boldsymbol{q})}{\partial \boldsymbol{q}} \boldsymbol{D} \frac{\partial \boldsymbol{\nu}(\boldsymbol{q}_{\mathrm{r}})}{\partial \boldsymbol{q}_{\mathrm{r}}} \dot{\boldsymbol{q}}_{\mathrm{r}} + \frac{\partial \boldsymbol{\omega}(\boldsymbol{q})}{\partial \boldsymbol{q}} \boldsymbol{f}\big(\boldsymbol{\nu}(\boldsymbol{q}_{\mathrm{r}})\big) &= \left.\frac{\partial \boldsymbol{\omega}(\boldsymbol{q})}{\partial \boldsymbol{q}} \boldsymbol{B} \boldsymbol{F}\right|_{\boldsymbol{q}=\boldsymbol{\nu}(\boldsymbol{q}_{\mathrm{r}})} \\
\boldsymbol{y}_{\mathrm{r}}(t) &= \boldsymbol{h}\big(\boldsymbol{\nu}(\boldsymbol{x}_{\mathrm{r}}(t))\big),
\end{aligned}
\end{equation}





\begin{equation} \label{eq:nonlin-ROM-nonlin-proj}
\begin{aligned}
\widetilde{\boldsymbol{M}}_{\mathrm{r}} \dot{\boldsymbol{q}}_{\mathrm{r}} + \frac{\partial \boldsymbol{\omega}(\boldsymbol{q})}{\partial \boldsymbol{q}} \boldsymbol{M} \frac{\partial^2 \boldsymbol{\nu}(\boldsymbol{q}_{\mathrm{r}})}{\partial \boldsymbol{q}_{\mathrm{r}}^2} \, \dot{\boldsymbol{q}}_{\mathrm{r}} \otimes \dot{\boldsymbol{q}}_{\mathrm{r}} + \widetilde{\boldsymbol{D}}_{\mathrm{r}} \dot{\boldsymbol{q}}_{\mathrm{r}} + \frac{\partial \boldsymbol{\omega}(\boldsymbol{q})}{\partial \boldsymbol{q}} \boldsymbol{f}\big(\boldsymbol{\nu}(\boldsymbol{q}_{\mathrm{r}})\big) &= \left.\frac{\partial \boldsymbol{\omega}(\boldsymbol{q})}{\partial \boldsymbol{q}} \boldsymbol{B} \boldsymbol{F}\right|_{\boldsymbol{q}=\boldsymbol{\nu}(\boldsymbol{q}_{\mathrm{r}})} \\
\boldsymbol{y}_{\mathrm{r}}(t) &= \boldsymbol{h}\big(\boldsymbol{\nu}(\boldsymbol{x}_{\mathrm{r}}(t))\big),
\end{aligned}
\end{equation}




\begin{equation*}
\resizebox{0.95\linewidth}{!}{
	$\dot{\boldsymbol{q}}_{\mathrm{r}}^v = \sum_{k=1}^{N} \boldsymbol{S}_v^{(k)} \, {\boldsymbol{q}_{\mathrm{r}}^{v}}^{(k)} = \boldsymbol{S}_{v}^{(1)} \boldsymbol{q}_{\mathrm{r}}^v + \boldsymbol{S}_{v}^{(2)} (\boldsymbol{q}_{\mathrm{r}}^v \otimes \boldsymbol{q}_{\mathrm{r}}^v) + \cdots $}
\end{equation*}
\begin{equation}
\resizebox{0.97\linewidth}{!}{
	$\ddot{\boldsymbol{q}}_{\mathrm{r}}^v = \sum_{k=1}^{N} \boldsymbol{S}_v^{(k)} \, {\dot{\boldsymbol{q}}_{\mathrm{r}}^{v}}^{(k)} = \boldsymbol{S}_{v}^{(1)} \boldsymbol{q}_{\mathrm{r}}^v + \boldsymbol{S}_{v}^{(2)} (\dot{\boldsymbol{q}}_{\mathrm{r}}^v \otimes \boldsymbol{q}_{\mathrm{r}}^v + \boldsymbol{q}_{\mathrm{r}}^v \otimes \dot{\boldsymbol{q}}_{\mathrm{r}}^v) + \cdots $}
\end{equation}
\begin{equation*}
\resizebox{0.95\linewidth}{!}{
	$\boldsymbol{F} = \sum_{k=1}^{N} \boldsymbol{R}^{(v)} {\boldsymbol{q}_{\mathrm{r}}^v}^{(k)} = \boldsymbol{R}^{(1)} \boldsymbol{q}_{\mathrm{r}}^v + \boldsymbol{R}^{(2)} (\boldsymbol{q}_{\mathrm{r}}^v \otimes \boldsymbol{q}_{\mathrm{r}}^v) + \cdots$}
\end{equation*}

==> tikz/nonlin-sys-nonlin-SG_steady-state-V.tex <==
\begin{tikzpicture}

  % Knoten / Blöcke
  \UeFunk[align = left, inner sep = 6 pt]{nonlinSigGen}{0, 0}{0.6 cm}{
		$\begin{aligned}
		\dot{\boldsymbol{q}}_{\mathrm{r}}^v(t) &= \boldsymbol{s}_{v}\big(\boldsymbol{x}_{\mathrm{r}}^v(t)\big) \\[0.2em]
		\ddot{\boldsymbol{q}}_{\mathrm{r}}^v(t) &= \frac{\partial \boldsymbol{s}_v\big(\boldsymbol{q}_{\mathrm{r}}^v(t)\big)}{\partial \boldsymbol{q}_{\mathrm{r}}^v(t)} \cdot \boldsymbol{s}_{v}\big(\boldsymbol{x}_{\mathrm{r}}^v(t)\big) \\[0.2em]
		\boldsymbol{F}(t) &= \boldsymbol{r}\big(\boldsymbol{q}_{\mathrm{r}}^v(t)\big)
		\end{aligned}$
  }
  \UeFunk[align = left, inner sep = 6 pt]{FOM}{6.7, 0}{0.6 cm}{
	    $\begin{aligned}
	    \boldsymbol{M} \ddot{\boldsymbol{q}}(t) + \boldsymbol{D} \dot{\boldsymbol{q}}(t) + \boldsymbol{f}\big(\boldsymbol{q}(t)\big) &= \boldsymbol{B} \boldsymbol{F}(t) \\[0.2em]
	    \boldsymbol{y}(t) &= \boldsymbol{C} \boldsymbol{q}(t)
	    \end{aligned}$
  } 
  \UeFunk[align = left, inner sep = 6 pt]{ROM}{6.7, -4}{0.6 cm}{
	  	$\begin{aligned}
     	\widetilde{\boldsymbol{M}}_{\mathrm{r}} \ddot{\boldsymbol{q}}_{\mathrm{r}} + \widetilde{\boldsymbol{g}} + \widetilde{\boldsymbol{D}}_{\mathrm{r}} \dot{\boldsymbol{q}}_{\mathrm{r}} + \widetilde{\boldsymbol{W}}(\boldsymbol{q})^{\mathsf T} \boldsymbol{f}\big(\boldsymbol{\nu}(\boldsymbol{q}_{\mathrm{r}})\big) &= \widetilde{\boldsymbol{B}}_{\mathrm{r}} \boldsymbol{F}\\
     	\boldsymbol{y}_{\mathrm{r}} &= \boldsymbol{C} \boldsymbol{\nu}\big(\boldsymbol{q}_{\mathrm{r}}\big)
     	\end{aligned}$
  }
  
  \Verzweigung{verzw-u}{2.5, 0}{3 pt}
  
  \Summationsstelle{summation}{11.5, 0}{0.4 cm}

   
  % Signalflüsse
  \draw[thick, -latex'] (nonlinSigGen) -- (FOM) node[pos = 0.49, above] {$\boldsymbol{u}(t)$};
  \draw[thick, -latex'] (verzw-u) |- (ROM);
  \draw[thick, -latex'] (FOM.east) -- (summation) node[pos = 0.76, above] {$\boldsymbol{y}(t)$};
  \draw[thick, -latex'] (ROM.east) -| (summation) node[pos = 0.25, above] {$\boldsymbol{y}_{\mathrm{r}}(t)$};
  \draw[thick, -latex'] (summation) -- (13.4, 0) node[pos = 0.49, above] {$\boldsymbol{e}(t)=\boldsymbol{0}$};
  
  \draw[thick, -latex'] (nonlinSigGen) -- + (0,1.7) node[pos = 0.7, right] {$\boldsymbol{q}_{\mathrm{r},0}^v \neq \boldsymbol{0}$} -- (nonlinSigGen);

  \draw[thick, -latex'] (FOM) -- + (0,1.7) node[pos = 0.7, right] {$\boldsymbol{q}_{0} = \boldsymbol{\nu}(\boldsymbol{q}_{\mathrm{r},0}^v)$} -- (FOM);
  
  \draw[thick, -latex'] (ROM) -- + (0,1.7) node[pos = 0.7, right] {$\boldsymbol{q}_{\mathrm{r},0} = \boldsymbol{\omega}(\boldsymbol{q}_{0})$} -- (ROM);

  % Beschriftungen
  \node[outer sep = 0.1 cm, below] at (nonlinSigGen.south) {\text{nonlinear signal generator}};
  \node[outer sep = 0.1 cm, below] at (FOM.south) {\text{FOM}};
  \node[outer sep = 0.1 cm, below] at (ROM.south) {\text{ROM}};
  
  \node[outer sep = 0.3 cm, below] at (summation.west) {$-\ $};
  
\end{tikzpicture}
